Data-driven dimensional analysis: algorithms for unique and relevant dimensionless groups

Classical dimensional analysis has two limitations: (i) the computed dimensionless groups are not unique, and (ii) the analysis does not measure relative importance of the dimensionless groups. We propose two algorithms for estimating unique and relevant dimensionless groups assuming the experimenter can control the system's independent variables and evaluate the corresponding dependent variable; e.g., computer experiments provide such a setting. The first algorithm is based on a response surface constructed from a set of experiments. The second algorithm uses many experiments to estimate finite differences over a range of the independent variables. Both algorithms are semi-empirical because they use experimental data to complement the dimensional analysis. We derive the algorithms by combining classical semi-empirical modeling with active subspaces, which---given a probability density on the independent variables---yield unique and relevant dimensionless groups. The connection between active subspaces and dimensional analysis also reveals that all empirical models are ridge functions, which are functions that are constant along low-dimensional subspaces in its domain. We demonstrate the proposed algorithms on the well-studied example of viscous pipe flow---both turbulent and laminar cases. The results include a new set of two dimensionless groups for turbulent pipe flow that are ordered by relevance to the system; the precise notion of relevance is closely tied to the derivative based global sensitivity metric from Sobol' and Kucherenko.

==> sec-import.tex <==
\section{Most important nondimensional numbers}

\subsection{Active subspaces}
\label{sec:asimport}

\noindent Active subspaces provide a natural and precise way to measure \emph{importance} among the variables. Recall the matrix that defines the active subspaces, given $f(\vx)$ and $\rho(\vx)$, and its eigenvalue decomposition,
\begin{equation}
\mC \;=\; \int \nabla_{\vx} f(\vx)\,\nabla_{\vx} f(\vx)^T\,\rho(\vx)\,d\vx \;=\; \mU\Lambda\mU^T.
\end{equation}
Define the rotated coordinates $\vy=\mU^T\vx$, and denote $\vy=[y_1,\dots,y_m]^T$. The density $\rho(\vx)$ induces a density $\sigma=\sigma(\vy)$ on $\vy$,
\begin{equation}
\sigma(\vy) \;=\; \rho(\mU\vy),
\end{equation}
since $\text{det}(\mU)=1$. Define a function of the rotated coordinates $g=g(\vy)$ as
\begin{equation}
g(\vy) \;=\; f(\mU\vy),
\end{equation}
and note its gradient with respect to $\vy$ is, by the chain rule,
\begin{equation}
\nabla_{\vy}g(\vy) \;=\; \nabla_{\vy} f(\mU\vy) \;=\; 
\mU^T\nabla_{\vx} f(\mU\vy).
\end{equation}
So each component of the gradient vector is
\begin{equation}
\frac{\partial}{\partial y_i}\,g(\vy) \;=\;
\vu_i^T\nabla_{\vx}f(\mU\vy),\qquad i=1,\dots,m,
\end{equation}
where $\mU=\bmat{\vu_1 &\cdots&\vu_m}$. 

The derivative-based sensitivity metric of Kucherenko and Sobol' provides a natural measure of \emph{importance} for the variables $\vy$ in the function $g(\vy)$; the metric for the $i$th variables is 
\begin{equation}
\int \left(\frac{\partial}{\partial y_i}\,g(\vy)\right)^2\,\sigma(\vy)\,d\vy,\qquad i=1,\dots,m.
\end{equation}
This number measures how much $g$ changes, on average, as $y_i$ is perturbed by a small amount. Observe that this metric is equal to the $i$th eigenvalue of $\mC$:
\begin{equation}
\begin{aligned}
& \int \left(\frac{\partial}{\partial y_i}\,g(\vy)\right)^2\,\sigma(\vy)\,d\vy\\
&\qquad
= \int \left( \vu_i^T\nabla_{\vx}f(\mU\vy) \right)^2\,\sigma(\vy)\,d\vy\\
&\qquad
= \int \left( \vu_i^T\nabla_{\vx}f(\mU\vy) \right)^2\,\rho(\mU\vy)\,d\vy\\
&\qquad
= \int \left( \vu_i^T\nabla_{\vx}f(\mU\mU^T\vx) \right)^2\,\rho(\mU\mU^T\vx)\,d\vx\\
&\qquad
= \int \left( \vu_i^T\nabla_{\vx}f(\vx) \right)
\left( \nabla_{\vx}f(\vx)^T\vu_i \right)
\,\rho(\vx)\,d\vx\\
&\qquad
= \vu_i^T\,
\left(\int \nabla_{\vx}f(\vx)\, \nabla_{\vx}f(\vx)^T\,\rho(\vx)\,d\vx\right)
\,\vu_i\\
&\qquad
= \vu_i^T\,\mC\,\vu_i \;=\; \lambda_i.
\end{aligned}
\end{equation}
Since the eigenvalues are ordered in descending order---i.e., $\lambda_i\geq\lambda_j$ for $i<j$---the components of $\vy$ are ordered according to their \emph{importance} as measured by the derivative-based sensitivity metric.

\subsection{Buckingham Pi}

\noindent Recall some of the concepts and terms from the Buckingham Pi analysis. The vector $\vw$ is defined as a solution to the linear system,
\begin{equation}
\mD\vw \;=\; \vv(q),
\end{equation}
where $q$ is the dimensional quantity of interest, $\vv(q)$ is its dimension vector, and $\mD$ is from \eqref{eq:D}. The $m\times n$ matrix $\mW=\bmat{\vw_1&\cdots&\vw_n}$ contains a basis for the null space of $\mD$,
\begin{equation}
\mD\,\mW \;=\; \mathbf{0}_{k\times n}.
\end{equation}
Let $\vx=\log(\vq)$, where $\vq=[q_1,\dots,q_m]^T$ are the dimensional inputs. Then the nondimensional quantity of interest is
\begin{equation}
\pi \;=\; q\,\exp(-\vw^T\vx),
\end{equation}
and the nondimensional inputs are
\begin{equation}
\pi_i \;=\; \exp(\vw_i^T\vx),\qquad i=1,\dots,n.
\end{equation}
The Buckingham Pi Theorem says that the physical law can be written in a nondimensional form as (see \eqref{eq:phi})
\begin{equation}
\pi \;=\; f(\pi_1,\dots,\pi_n).
\end{equation}
Create a new set of set of variables for the nondimensional law,
\begin{equation}
\label{eq:gg}
\begin{aligned}
\pi 
&= f(\pi_1,\dots,\pi_n)\\
&= f\big(
\exp(\log(\pi_1)),\dots,\exp(\log(\pi_n))
\big)\\
&= g\big(
\log(\pi_1),\dots,\log(\pi_n)
\big)\\
&= g(\gamma_1,\dots,\gamma_n),
\end{aligned}
\end{equation}
for a function $g:\mathbb{R}^n\rightarrow\mathbb{R}$.

\subsection{The most important nondimensional parameter}

\noindent We need a density function on the new variables $\bgamma=[\gamma_1,\dots,\gamma_n]^T$ to apply active subspaces to the nondimensional law. Note that, for $\bpi=[\pi_1,\dots,\pi_n]^T$,
\begin{equation}
\bgamma \;=\; \log(\bpi) \;=\; \mW^T\vx \;=\; \mW^T\log(\vq).
\end{equation}
Therefore, a joint density function on the dimensional quantities $\vq$ or their logs $\log(\vq)$ induces a joint density function on $\bgamma$, which we denote $\rho(\bgamma)$. Assume that $g$ from \eqref{eq:gg} satisfies the conditions needed to get active subspaces (i.e., differentiable and square integrable derivatives with respect to $\rho(\bgamma)$). Then active subspaces for the nondimensional law can be constructed from the eigendecomposition
\begin{equation}
\label{eq:Cg}
\int \nabla_{\bgamma}g(\bgamma)\, \nabla_{\bgamma}g(\bgamma)^T\,\rho(\bgamma)\,d\bgamma
\;=\; \mU\Lambda\mU^T.
\end{equation}
As in Section \ref{sec:asimport}, we define a new set of coordinates $\bdelta=[\delta_1,\dots,\delta_n]^T$ by the rotation $\mU$ that are ordered by \emph{importance}---where importance is defined by the derivative-based sensitivity metrics. Let $\bdelta=\mU^T\bgamma$, and define the function $h=h(\bdelta)$ as
\begin{equation}
h(\bdelta) \;=\; g(\mU\bdelta).
\end{equation}
Assume that there is strict separation between the first two eigenvalues from \eqref{eq:Cg}, i.e., $\lambda_1>\lambda_2$. For the first eigenvector $\vu_1$,
\begin{equation}
\delta_1 
\;=\; \vu_1^T\bgamma\\
\;=\; \vu_1^T\mW^T\vx\\
\;=\; \vz_1^T\vx,
\end{equation}
where $\vz_1=\mW\vu_1$. Then the most important nondimensional quantity for the physical law is
\begin{equation}
\exp(\delta_1) \;=\; \exp(\vz_1^T\vx) \;=\; \exp\left(\vz_1^T\log(\vq)\right).
\end{equation}
More generally, we see that $\bdelta$ defines an ordering of nondimensional parameters---assuming strict separation of the eigenvalues in \eqref{eq:Cg}. In other words, if $\lambda_i>\lambda_j$ for $i<j$, then the nondimensional numbers
\begin{equation}
\label{eq:z}
\exp\left(\vz_i^T\log(\vq)\right),\quad \vz_i=\mW\vu_i,\quad i=1,\dots,n,
\end{equation}
are ordered from most important to least important. To see that these numbers are nondimensional, note
\begin{equation}
\mD\vz_i \;=\; \mD\mW\vu_i \;=\; \left[\mathbf{0}_{k\times n}\right]\,\vu_i \;=\; \mathbf{0}_{k\times 1}.
\end{equation}
In words, $\vz_i$ is in the null space of $\mD$, so it defines a nondimensional parameter. It is a simple exercise to show that---under strict separation in the eigenvalues---these nondimensional parameters are unique. To do this, replace the basis $\mW$ for the null space of $\mD$ by a rotated basis $\mW\mQ$, where $\mQ\in\mathbb{R}^{n\times n}$ is orthogonal. 

\subsection{Numerically approximating the important nondimensional parameters}

\noindent There are two ways (that I can think of) to estimate the $\vz_i$ that define the ordered-by-importance nondimensional parameters.

\subsubsection{Approximating $g$ with a response surface}

\noindent Given vectors $\vw$ and $\vw_1,\dots,\vw_n$ that define the nondimensional quantity of interest and initial nondimensional parameters, respectively. And given samples $(q^{(j)},\vq^{(j)})$ with $j=1,\dots,N$ that correspond to $N$ ``experiments,'' where $\vq^{(j)}$ are drawn according to a given density on $\vq$ or $\log(\vq)$. 
\begin{enumerate}
\item Compute samples of the nondimensional quantity of interest
\begin{equation}
\pi^{(j)} \;=\; q^{(j)}\,\exp\left(-\vw^T\log(\vq^{(j)})\right)
\end{equation}
\item Compute samples of the logs of the nondimensional parameters
\begin{equation}
\gamma_i^{(j)} \;=\; \vw_i^T\log(\vq^{(j)}), \qquad i=1,\dots,n,
\end{equation}
and $\bgamma^{(j)}=[\gamma_1^{(j)},\dots,\gamma_n^{(j)}]^T$.
\item Fit a model (e.g., a least-squares-fit polynomial) $\hat{g}$ with the pairs $(\pi^{(j)},\bgamma^{(j)})$ such that
\begin{equation}
\pi^{(j)} \;\approx\; \hat{g}(\bgamma^{(j)}).
\end{equation}
\item Use the gradient $\nabla_{\bgamma}\hat{g}$ to define active subspaces:
\begin{equation}
\int \nabla_{\bgamma} \hat{g}(\bgamma)\, \nabla_{\bgamma} \hat{g}(\bgamma)^T\,\rho(\bgamma)\,d\bgamma
\;=\; \mU\Lambda\mU^T.
\end{equation}
Estimate these integrals with Monte Carlo or some other multivariate integration rule.
\item Compute the weights $\vz_i$ that define the important nondimensional quantities (see \eqref{eq:z}),
\begin{equation}
\vz_i \;=\; \mW\vu_i, \qquad i=1,\dots,n.
\end{equation}
\end{enumerate}
The trouble with this approach is the need to fit $\hat{g}$, which is always an issue if $n$ is large. 

A related approach may use statistical methods for sufficient dimension reduction with the pairs $(\pi^{(j)}, \bgamma^{(j)})$. However, in this case the precise sense of \emph{importance} would be different. 

\subsubsection{Finite difference gradients}

\noindent The idea here is to try to estimate the gradients of $g$ without building a global model. Instead, since we want local gradient information over the support of $\rho(\bgamma)$. So we can use finite differences at several points in space. The first two steps below are the same as the algorithm above. From there, the idea is to estimate gradients with finite differences. Step 3 is the most interesting.

Given vectors $\vw$ and $\vw_1,\dots,\vw_n$ that define the nondimensional quantity of interest and initial nondimensional parameters, respectively. And given samples $(q^{(j)},\vq^{(j)})$ with $j=1,\dots,N$ that correspond to $N$ ``experiments,'' where $\vq^{(j)}$ are drawn according to a given density on $\vq$ or $\log(\vq)$.
\begin{enumerate}
\item Compute samples of the nondimensional quantity of interest
\begin{equation}
\pi^{(j)} \;=\; q^{(j)}\,\exp\left(-\vw^T\log(\vq^{(j)})\right)
\end{equation}
\item Compute samples of the logs of the nondimensional parameters
\begin{equation}
\gamma_i^{(j)} \;=\; \vw_i^T\log(\vq^{(j)}), \qquad i=1,\dots,n,
\end{equation}
and $\bgamma^{(j)}=[\gamma_1^{(j)},\dots,\gamma_n^{(j)}]^T$.
\item For each $\bgamma^{(j)}$, find $\vq^{(j,k)}$ that satisfy
\begin{equation}
\mW^T\log(\vq^{(j,k)}) = \bgamma^{(j)} + h\,\ve_k,\qquad k=1,\dots,n,\quad j=1,\dots,N,
\end{equation}
where $\ve_k$ is a vector of zeros except for a 1 in the $k$th element and $h$ is the step size. These are the points used to compute finite differences. Note that these points are not unique (since the system of equations is underdetermined), but the nonuniqueness does not impact the results. 
\item For each $\vq^{(j,k)}$, run an ``experiment'' to get the corresponding quantity of interest $q^{(j,k)}$. 
\item Compute the corresponding nondimensional quantities
\begin{equation}
\pi^{(j,k)} \;=\; q^{(j,k)}\,\exp\left(-\vw^T\log(\vq^{(j,k)})\right)
\end{equation}
\item Compute finite differences
\begin{equation}
\frac{\partial}{\partial \gamma_k} g(\bgamma^{(j)})
\;\approx\; \frac{1}{h}(\pi^{(j,k)} - \pi^{(j)}),
\end{equation}
and let $\nabla_{\bgamma}'g(\bgamma^{(j)})\in\mathbb{R}^n$ be the collection of finite difference partial derivatives. 
\item Estimate the active subspaces as
\begin{equation}
\frac{1}{N}\sum_{j=1}^N \nabla_{\bgamma}'g(\bgamma^{(j)})\, \nabla_{\bgamma}'g(\bgamma^{(j)})^T \;=\; \mU\Lambda\mU^T. 
\end{equation}
One could use a different multivariate integration rule depending on how one chooses the points $\bgamma^{(j)}$.
\item Compute the weights $\vz_i$ that define the important nondimensional quantities (see \eqref{eq:z}),
\begin{equation}
\vz_i \;=\; \mW\vu_i, \qquad i=1,\dots,n.
\end{equation}
\end{enumerate}
The issue with this approach is the number $N(n+1)$ of ``experiments'' needed to estimate the finite differences. An approach similar to Constantine, Eftekhari, and Wakin (2015) may be used to cut down on the number of necessary experiments. 

